Size-adaptive Hypothesis Testing for Fairness

Determining whether an algorithmic decision-making system discriminates against a specific demographic typically involves comparing a single point estimate of a fairness metric against a predefined threshold. This practice is statistically brittle: it ignores sampling error and treats small demographic subgroups the same as large ones. The problem intensifies in intersectional analyses, where multiple sensitive attributes are considered jointly, giving rise to a larger number of smaller groups. As these groups become more granular, the data representing them becomes too sparse for reliable estimation, and fairness metrics yield excessively wide confidence intervals, precluding meaningful conclusions about potential unfair treatments. In this paper, we introduce a unified, size-adaptive, hypothesis-testing framework that turns fairness assessment into an evidence-based statistical decision. Our contribution is twofold. (i) For sufficiently large subgroups, we prove a Central-Limit result for the statistical parity difference, leading to analytic confidence intervals and a Wald test whose type-I (false positive) error is guaranteed at level $\alpha$. (ii) For the long tail of small intersectional groups, we derive a fully Bayesian Dirichlet-multinomial estimator; Monte-Carlo credible intervals are calibrated for any sample size and naturally converge to Wald intervals as more data becomes available. We validate our approach empirically on benchmark datasets, demonstrating how our tests provide interpretable, statistically rigorous decisions under varying degrees of data availability and intersectionality.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{NeurIPS Paper Checklist}

\begin{comment}
%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 
\end{comment}
%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the claims made in the abstract and introduction accurately reflect the paper's contributions and scope. We provide the theoretical framework for hypothesis testing for fairness in \cref{sec:framework} and empirical results in \cref{sec:experiments}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Limitations of the work are discussed in the Conclusions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detail the assumption of theoretical results in \cref{sec:framework}. We formally prove our results in the Supplementary Material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper describes how experiments were run at a high level in \S\ref{sec:data-models}, while the specific details to reproduce the results are described in the Supplementary Material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code and data are available in the Supplementary Material, and instructions to reproduce the results are given.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The Experiments Section describes how many data splits were used for the results, and details about the models used, even though they are not a central part of the results, are included in the Supplementary Material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report the results across all the train-test splits. Furthermore, we report confidence/credible intervals as correctly produced via central limit results or bayesian inference.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Reproducibility in \S\ref{sec:data-models} provides the computational resources needed to reproduce the experiments, and, while running the experiments only takes a few minutes, more details are provided in the Supplementary Material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We followed the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Broader impacts are discussed in the Conclusions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not foresee any high risk for misuse of this work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we credited them in appropriate ways.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We used LLMs only for editing/formatting.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> exp_notes.tex <==

We conducted multiple experiments to analyze the methodologies outlined in Section~\ref{sec:framework}. Using our framework, we assessed fairness in intersectional settings and explored the additional insights it provides to stakeholders regarding the fairness-aware implementation of machine learning models.
\inote{pointer to supplementary}
%For both we consider a binary classification problem, use as predictive model an XGBoost \citep{XGBoost}, and identify the protected variables among the features available in the dataset. For both datasets the identified protected variables are \textit{race}, \textit{age} and \textit{sex}. We proceed to evaluate fairness in terms of Statistical Parity by gradually increasing the number of the protected variables, and thus the level of intersectionality. Thus, we start by considering only the subgroups relative to the protected variables (\textit{race}, \textit{age} and \textit{sex}), then the paired protected variables (\textit{race and age}, \textit{race and sex}, \textit{age and sex}), and lastly all the intersectional subgroups. 


\subsection{COMPAS}


\paragraph{Methodology}
We select for our experiments 8 features that include the count of juvenile felonies and misdemeanors, prior counts, charge degree (felony or misdemeanor), and whether the individual was recidive within two years or not. We encode all features as categorical, with the exception of prior counts. 
The predictor $g : \mathcal{X} \rightarrow \mathcal{Y}$ (a XGBoost model) is trained on $x \in \mathcal{X}_{train}$ to predict whether the individual might reoffend within two years ($y = 1$) or not ($y = 0$). 



The protected variables and their values are:
{\small
\begin{itemize}
    \item "African-American", "Asian", "Caucasian", "Hispanic", "Native American", "Other" $\in S_{race}$
    \item "Under 25", "25-45", "Over 45" $\in S_{age}$
    \item "Female", "Male" $\in S_{sex}$
\end{itemize}
}

%The predictor $g : \mathcal{X} \rightarrow \mathcal{Y}$ (a XGBoost model) is trained on the datapoint of the training $x \in \mathcal{X}_{train}$, to predict whether the individual might reoffend within two years ($y = 1$) or not ($y = 0$). 

We gradually increase the level of intersectionality for the analysed groups. Thus, we start by considering only the non-intersectional subgroups (\textit{race}, \textit{age} and \textit{sex}), then the groups at the intersection of two or three protected variables.% (\textit{race and age}, \textit{race and sex}, \textit{age and sex}), and lastly all the intersectional subgroups. 
We proceed to evaluate fairness in terms of SP (Eq.~\ref{eq:sp}), $\delta$SP (Eq.~\ref{eq:delta-sp}), $\gamma$SP (Eq.~\ref{eq:gamma-sp}), and our STF (Algorithm~\ref{algo}), and compare the results.

%We consider as $s$ an element belonging to either $S_{race}$, $S_{age}$, $S_{sex}$, $S_{race} \times S_{age}$, $S_{race} \times S_{sex}$, $S_{age} \times S_{sex}$ and $S_{race} \times S_{age} \times S_{sex}$ and as $\bar{S}$ any group different from $s$. 



%We want to assess the fair treatment of individuals by a predictive model $g$ trained on the Adult Income and the COMPAS datasets in terms of statistical parity $SP$ over the intersectional subgroups $s$ of the protected variables in the datasets. 

%A point-wise estimate of $SP$ is not enough to determine whether or not a subgroup of individuals is being advantaged or disadvantaged by the predictive model. $SP(s)$ could in fact be just slightly above or below the fair value of 0. Normally, one would have to choose a value $\delta$ of tolerance and flag unfair treatment of a subgroup $s$ if $|SP(s)| > \delta$. However, this is an arbitrary choice that experts have to make, and it does not take into account the number of samples over which we are estimating $SP(s)$ or the level of certainty one has over the value $SP(s)$. We could have an estimated value of $SP(s)$ fairly above or below 0, but with a confidence interval so large that it does include the fair value of 0 in it. In such a case, we could say that under that level of confidence, the subgroup $s$ is not being treated unfairly. We could also have an estimated value of $SP(s)$ very close to 0, but with a very small confidence interval that does not include the fair value of 0 in it. In such a case, we could say that under that level of confidence, the subgroup $s$ is being treated unfairly. In Subsection 4.1, we show how to theoretically determine the asymptotic behaviour of statistical parity, and how to estimate $SP(s)$ and its confidence interval when the number of samples $n \rightarrow \infty$. In Section 4.2, we covered how to estimate $SP(s)$ and its confidence interval when the number of samples is small by using a Bayesian inference approach. We first look at the results of the estimations of $SP(s)$ and its confidence value using both approaches on the predictions of the predictive models $g$ on the test sets of the Adult Income and COMPAS datasets, and see when the two approaches converge and when they do not. Then, we proceed by assessing the fairness treatment of the subgroups $s$ in the two datasets using our methodologies. Thus, if $SP(s) - CI \leq 0 \leq SP(s) + CI $ we say that the subgroup $s$ is treated fairly by the predictive model under the level of confidence $CI$, otherwise we flag the subgroup $s$ as being treated unfairly by the model. We compare at different levels of intersectionality what conclusions we might get by using our approach. Then, we compare the findings using our approach with the $\delta$-Statistical parity approach, and the $\gamma$-Statistical approach, and discuss under what conditions we get fairly similar results. Lastly, we discuss how our approach can make the assessment of fair treatment of individuals by predictive ML models easier, more straight-forward, and how it can provide more information to stakeholders compared to previous approaches.  

\paragraph{Results}
In this context, the statistical parity difference quantifies the disparity in prediction outcomes between individuals in the protected subgroup $S$ and those in the complementary group $\bar{S}$. Specifically, it measures the difference in probabilities of being predicted by $g$ to reoffend within two years, highlighting whether the protected group is advantaged or disadvantaged relative to the rest of the population.
%In this context, the statistical parity difference (Eq.~\ref{eq:sp})
%\[
%SP(S) = \mathbb{P}(g(x)=1|s \in S) - \mathbb{P}(g(x)=1|s \in \bar{S})
%\]
%represents how higher (or lower) is compares the probability for individuals belonging to the protected subgroup $s$ to be predicted by $g$ to reoffend within two years with the same prob for the other group. 
If $\mathrm{SP}(S) > 0$, the subgroup $s$ is \textit{advantaged} compared to the rest of the population $\bar{S}$, if $\mathrm{SP}(S) < 0$ the subgroup $S$ is \textit{disadvantaged}. 

In Figure~\ref{fig:cherrypick_compas} we select three intersectional groups, respectively (Caucasian, Male) (leftmost panel), (Native American, Female) (center) and (African American, Male, 25-45) (right). We fold the dataset in different ways and observe the impact on the SP. For each split we compute the point-wise SP estimation, the bayesian (blue) and the asymptotic (red) confidence interval.
In Figure~\ref{fig:cherrypick_compas}(left) traditional approaches would not have detected a fairness violation, while with out approach we do so for all splits, since the confidence interval excludes zero and we can reject the null hypothesis. In Figure~\ref{fig:cherrypick_compas}(center) we observe how in all cases the asymptotic evaluation converges to the point estimation. In this case fixed-threshold-based approaches would have reported a fairness violation, but we cannot reject the null hypothesis. The missing lines in the central panel are due to splits that did not include any point ($n_{min}=0$). Figure~\ref{fig:cherrypick_compas}(right) is somewhat specular to Figure~\ref{fig:cherrypick_compas}(center), but in this case the polarity of the fairness violation is disadvantageous for the group.


In Figure \inote{GET GAMMA W BARS} 
The horizontal axis displays the number of samples for each intersectional group, while on the vertical axis we report the value of $\gamma$-statistical parity value for that group. In red the groups that are flagged for unfairness and in blue those that are not. \itodo{TODO: write what should we conclude. Essentially that with a threshold we can not achieve ours classification, hence it is imprecise(?)}

\subsection{Adult}


\paragraph{Methodology}
 We encode the categorical features with a LabelEncoder, and scale with a StandardScaler the numerical features. We proceed to split the dataset of 48842 datapoints into a training set of 36631 samples (roughly 75\% of the total) and a test set of 12211 samples (roughly 25\% of the total). We identify as sets of protected variables $s$ that should not be provided to the predictive model: $S_{race}$, $S_{age}$ and $S_{sex}$. Regarding \textit{age}, which is a numerical feature of the dataset, we group it into four age groups: under 18, 18 to 40, 40 to 65, and over 65. Thus, the subgroups for the three protected variables are:
\warning{Here we should better define/contextualize $X$ (Maybe we can simply use lower case $x$, or define the associated random variable X. Also, we need to decide what to do with S and definition of protected groups}
\begin{itemize}
    \item "Amer-Indian-Eskimo", "Asian-Pacific-Islander", "Black", "Other", "White" $\in S_{race}$
    \item "Under 18", "18 to 40", "40 to 65", "Over 65" $\in S_{age}$
    \item "Female", "Male" $\in S_{sex}$
\end{itemize}
The predictor $g : \mathcal{X} \rightarrow \mathcal{Y}$ (a XGBoost model) is trained on the datapoint of the training $x \in \mathcal{X}_{train}$, to predict whether the individual income is above \$50k per year ($y = 1$) or not ($y = 0$). We consider as $s$ an element belonging to either $S_{race}$, $S_{age}$, $S_{sex}$, $S_{race} \times S_{age}$, $S_{race} \times S_{sex}$, $S_{age} \times S_{sex}$ and $S_{race} \times S_{age} \times S_{sex}$ and as $\bar{S}$ any group different from $s$. In this context, the statistical parity difference
\[
SP(s) = \mathbb{P}(g(x)=1|s \in S) - \mathbb{P}(g(x)=1|x \in \bar{S})
\]
represents how higher (or lower) is the probability for individuals belonging to the protected subgroup $s$ to be predicted by $g$ to have an annual income above \$50k per year. If $SP(s) > 0$, the subgroup $s$ is \textit{advantaged} compared to the rest of the population $\bar{S}$, if $SP(s) < 0$ the subgroup $s$ is \textit{disadvantaged}. 

\paragraph{Results}


\subsection{Student}

TBC

\paragraph{Methodology}
\paragraph{Results}



\paragraph{Adult}


\paragraph{COMPAS}

\paragraph{Overview}


\paragraph{Comparison theoretical and bayesian approach} 

Here we discuss some example of when it converges well and when it does not, picked examples of unfair treatment with little confidence interval, and cases with fair treatment with large confidence intervals

\paragraph{Flagging over intersections}


\paragraph{$\delta$-SP}

Here we discuss results with $\delta$-SP




\paragraph{$\gamma$-SP}

Here we discuss results with $\gamma$-SP.




\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figs/experiments/adult_case_1_1.pdf}
        \caption{Our method says unfair, traditional does not}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figs/experiments/adult_case_2_1.pdf}
        \caption{Traditional would say unfair, we know too imprecises}
        \label{fig:sub2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.28\textwidth}
        \includegraphics[width=\textwidth]{figs/experiments/adult_case_3_1.pdf}
        \caption{Traditional and our method agree it's unfair}
        \label{fig:sub3}
    \end{subfigure}
    \caption{Adult anecdotal: In blue bayesian, in red asymptotic}
    \label{fig:main}
\end{figure}


==> relwork.tex <==
\section{Background and Related Work}

Early research on algorithmic fairness framed the problem as ensuring statistical parity across sensitive groups defined by single attributes such as race or gender.  Demographic Parity~\citep{feldman2015certifying}, Equalized Odds and Equal Opportunity~\citep{hardt2016equality}, Predictive Parity~\citep{chouldechova2017fair}, and related criteria remain cornerstones of the field and are implemented in popular toolkits (e.g., \textsc{Fairlearn}~\citep{weerts2023fairlearn}).  A large body of work subsequently proposed pre‑, in‑, and post‑processing interventions to satisfy one or more of these metrics~\citep{zafar2017fairness, friedler2019comparative}. \textbf{Motivation, integrabile in intro} 

While the above metrics are ordinarily reported as single numbers, they are in fact noisy estimates computed on finite samples.  \citet{angwin2022machine} and the ensuing debate around COMPAS highlighted how small data perturbations can flip an “unfair’’ judgment.  \citet{kearns2018preventing} observed that even with large overall data sets, fairness estimates for minority sub‐groups can have extremely high variance, a problem magnified under intersectionality.  Recent surveys \citep{besse2022survey,bhatt2021uncertainty} consolidate evidence that ignoring estimation error leads to both false alarms (flagging random fluctuation as bias) and missed harms (overlooking small but significant disparities in large groups). \textbf{Motivation (focus on metrics), integrabile in intro} 
% Different studies have shown that treating single‑sample estimates as ground truth can flip a fair/unfair verdict under minor data perturbations.  Building on this critique, \citet{lim2022fourfifths} demonstrate both theoretically and empirically that the ubiquitous “four‑fifths rule’’ (80\% disparate‑impact threshold) has poor statistical power and yields high false‑positive and false‑negative rates, especially for small or imbalanced groups.  Their results reinforce the need to replace fixed thresholds with uncertainty‑aware evaluation.

Intersectionality~\citep{crenshaw2013demarginalizing,Gohar2023ASO} demands analysis at the cross‑sections of multiple protected attributes (e.g.\ “Black women over 50’’).  Empirical studies such as \textit{Gender Shades}~\citep{buolamwini2018gender} revealed accuracy gaps that only appear at such intersections.  Yet the number of subgroups grows exponentially with attribute count, leaving most groups sparsely represented.
\citet{foulds2020intersectional} formalised this “resolution limit’’ and demonstrated that point estimates become statistically meaningless in the low‑data regime.
Subsequent work proposed auditing algorithms that search adaptively for large‑effect subgroups without exhaustively enumerating all intersections~\citep{kearns2018preventing, morina2019auditing}, but these methods still deliver binary verdicts on noisy estimates. 
%
%
% Subsequent Bayesian approaches borrow strength across groups to stabilise estimates~\citep{foulds2020bayesian}.
Complementary to these estimation strategies, \citet{molina2022bounding} provide high‑probability \emph{bounds} that connect easily measured \emph{marginal} fairness to otherwise intractable intersectional fairness.  Their analysis shows when marginal guarantees suffice and offers computable certificates that scale to many attributes.
%
% Intersectionality demands analysis at the cross‑sections of multiple protected attributes, yet the exponential blow‑up in subgroup count leaves most intersections too sparse for reliable estimation.  \citet{foulds2020intersectional} formalised this “resolution limit,’’ and subsequent Bayesian approaches borrow strength across groups to stabilise estimates~\citep{foulds2020bayesian}.  Complementary to these estimation strategies, \citet{molina2022bounding} provide high‑probability \emph{bounds} that connect easily measured \emph{marginal} fairness to otherwise intractable intersectional fairness.  Their analysis shows when marginal guarantees suffice and offers computable certificates that scale to many attributes. 
 \textbf{Motivation (focus on intersectionality), integrabile in intro} 

A direct frequentist remedy is to report confidence intervals (CIs) around each fairness metric.  Bootstrap CIs for Demographic Parity, Equalized Odds, and related metrics are supported in \textsc{Fairlearn} and have been advocated by \citet{besse2018confidence}, \citet{del2019central}, and \citet{cherian2024statistical}. 
In NLP, \citet{ethayarajh-2020-classifier} introduce \emph{Bernstein‑bounded unfairness}, deriving analytic Bernstein bounds that convert a small, partially annotated sample into a tight confidence interval on bias.
Wide intervals immediately signal when data are insufficient to draw conclusions, a property exploited in the \textit{FairlyUncertain} benchmark~\citep{barrainkua2024uncertainty}. Nevertheless, CIs provide only marginal improvements when sample sizes are extremely small. % and must be recomputed each time the metric of interest changes. 
 \textbf{Non so mi sembra che sminuisca un po' il nostro} 

Bayesian models encode uncertainty through posterior distributions rather than fixed intervals.  \citet{dimitrakakis2019bayesian} introduced a Bayesian decision‑theoretic framework that trades off expected utility and expected unfairness under parameter uncertainty.  For intersectional analysis, hierarchical Bayes can “borrow strength’’ across related groups: \citet{foulds2020bayesian} show more stable bias estimates for rare intersections by sharing information via group‑level priors.  Bayesian methods have also been used to compare competing models under uncertainty~\citep{ji2020can} and to learn fair personalised rankers ~\citep{ngaffo2023fairbayrank}.  Practical uptake remains limited, however, due to sensitivity to prior specification and the computational burden of posterior inference. \textbf{I più importanti di bayesian gli ho messi nell'intro} 

Beyond estimating metrics more precisely, several authors treat disparities in predictive uncertainty themselves as indicators of unfairness.  \citet{bhatt2021uncertainty} decompose aleatoric and epistemic uncertainty across groups; higher epistemic uncertainty for a subgroup suggests under‑representation in the training data.  \citet{kuzucu2024uncertainty} leverage uncertainty estimates from deep ensembles and Bayesian neural networks to design uncertainty‑aware mitigation strategies. \textbf{probably on appendix} 
% The open challenge is to integrate such second‑order information with conventional fairness objectives.

Existing solutions thus improve fairness assessment along isolated axes--frequentist intervals or Bayesian posteriors--but none provides a unified, scalable framework that (i) quantifies estimation uncertainty, (ii) adapts gracefully to the extreme sparsity of intersectional subgroups, and (iii) remains agnostic to the choice of fairness metric.  We address this gap by introducing a statistically principled method that merges hierarchical Bayesian modelling with concentration‑inequality guarantees, yielding valid uncertainty bounds at small subgroup granularity without prohibitive computation. \textbf{General, can go in intro} 
% Empirically, our approach delivers decisive gains over prior CI‑based and Bayesian baselines, particularly in the low‑sample intersectional regime.

% \subsection{Still to be included}

% \textbf{Fairness in genera}l

% \cite{romei2014multidisciplinary}  A multidisciplinary survey on discrimination analysis.

% \cite{kamiran2010discrimination} Discrimination aware decision tree learning.

% \cite{roh2021sample} Neurips: Sample selection for fair and robust training

% \cite{meding2024fairness}:
% Describes the growing impact of machine learning algorithms and their potential for discriminatory behavior.
% Mentions the importance of fairness in machine learning and the challenges in defining and quantifying it.
% Highlights the focus on biased training data as a cause of discriminatory outcomes.
% Notes the connection between fairness and privacy in machine learning

% \textbf{Fairness measures and definitions}

% \cite{Kleinberg2016InherentTI} (differences in  calibration and balance) Inherent Trade-Offs in the Fair Determination of Risk Scores

% \textbf{Fairness and Uncertainty}
%
% \cite{bhatt2021uncertainty} Uncertainty as a form of transparency: Measuring, communicating, and using uncertainty
%
% \cite{barrainkua2024uncertainty} Uncertainty matters: stable conclusions under unstable assessment of fairness results.
%
% \cite{kuzucu2023uncertainty} Uncertainty-based fairness measures,
% \cite{kuzucu2024uncertainty} Uncertainty as a Fairness Measure. Uncertainty is on the predicted proba.
%
% \cite{ethayarajh-2020-classifier} Is Your Classifier Actually Biased? Measuring Fairness under Uncertainty with Bernstein Bounds


% \textbf{Intersectionality}
%
% \cite{Gohar2023ASO} A Survey on Intersectional Fairness in Machine Learning: Notions, Mitigation, and Challenges

% \cite{kearns2018preventing} Preventing fairness gerrymandering: Auditing and learning for subgroup fairness

% \cite{cherian2024statistical} Statistical inference for fairness auditing: "We show how the bootstrap can be used to simultaneously bound performance disparities over a collection of groups with statistical guarantees"


% \textbf{Relevant}
%
% \cite{foulds2020bayesian} Bayesian Modeling of Intersectional Fairness: The Variance of Bias. There is a wide difference here, as the want to calculate a threshold ($\gamma$ in their paper) such that the difference in statistical parity is below this gamma for all the possible intersectional groups. They do not provide confidence intervals for the actual fairness metric.
%
% \cite{foulds2020intersectional} An intersectional definition of fairness. (same author similar as above)
%
% \cite{ji2020can} Can I Trust My Fairness Metric? Assessing Fairness with Unlabeled Data and Bayesian Inference. They focus on unlabeled data and not on small intersectional groups. Metareview: The significance of the contribution (an auditor tool only, instead of an auditor plus a mitigation tool) is however at the low side.
%
% Inferential setting: \cite{besse2018confidence}, Confidence intervals for testing disparate impact in fair learning. \cite{besse2022survey} the published version of the previous one. \cite{del2019central}
% A central limit theorem for 
% transportation cost on the real line with application to fairness assessment in machine learning.
%
% \cite{molina2022bounding} Bounding and approximating intersectional fairness through marginal fairness.


%\section{Definitions}

%Definition of Subgroup Fairness, according to~\cite{Gohar2023ASO}:

%Let $\mathcal{C}=\{c: \mathcal{X}\rightarrow\{0,1\}\}$ be a collection of characteristic functions  where $c(s)=1$ indicates that an individual with protected attribute $s$ is in subgroup $c$.

%\begin{definition} 
%\textit{$f(x)$ is $\gamma-$SP subgroup fair if $\forall$ $c \in \mathcal{C}$:}
%   $$|P(f(x) = 1) - P(f(x) = 1 | c(s) = 1)| 
%    \times P(c(s) = 1) \leq \gamma,$$
%\end{definition}

%In this case, the $\gamma$-SP is determined by the worst-case group $c \in \mathcal{C}$. 

%From the paper: "The second term reweighs the difference by the proportion of the size of each subgroup in relation to the population. Consequently, the unfairness of smaller-sized groups is down-weighted in the final $\gamma-$SP estimation. \textit{Thus, it may not adequately protect small subgroups, even if they have high levels of unfairness.}"

